A Spitzer Space Telescope survey of extreme Asymptotic Giant Branch stars in M32

We investigate the population of cool, evolved stars in the Local Group dwarf elliptical galaxy M32, using Infrared Array Camera observations from the Spitzer Space Telescope. We construct deep mid-infrared colour-magnitude diagrams for the resolved stellar populations within 3.5 arcmin of M32's centre, and identify those stars that exhibit infrared excess. Our data is dominated by a population of luminous, dust-producing stars on the asymptotic giant branch (AGB) and extend to approximately 3 mag below the AGB tip. We detect for the first time a sizeable population of `extreme' AGB stars, highly enshrouded by circumstellar dust and likely completely obscured at optical wavelengths. The total dust-injection rate from the extreme AGB candidates is measured to be $7.5 \times 10^{-7}$ ${\rm M}_{\odot} \, {\rm yr}^{-1}$, corresponding to a gas mass-loss rate of $1.5 \times 10^{-4}$ ${\rm M}_{\odot} \, {\rm yr}^{-1}$. These extreme stars may be indicative of an extended star-formation epoch between 0.2 and 5 Gyr ago.

==> aasymbols.tex <==
% Astronomy and Astrophysics symbol macros (from aa.cls and mnras.cls)

\def\la{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\sim\cr}}}}}

\def\ga{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\sim\cr}}}}}

\newcommand\getsto{\mathrel{\mathchoice {\vcenter{\offinterlineskip
\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr\gets\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
\gets\cr\to\cr}}}}}

\newcommand\cor{\mathrel{\mathchoice {\hbox{$\widehat=$}}{\hbox{$\widehat=$}}
{\hbox{$\reset@font\scriptstyle\hat=$}}
{\hbox{$\reset@font\scriptscriptstyle\hat=$}}}}

\newcommand\lid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr<\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr<\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr<\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
<\cr
\noalign{\vskip0.9pt}=\cr}}}}}

\newcommand\gid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr>\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr>\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr>\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
>\cr
\noalign{\vskip0.9pt}=\cr}}}}}

\newcommand\sol{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr\sim\cr<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
\sim\cr<\cr}}}}}

\newcommand\sog{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr\sim\cr
>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
\sim\cr>\cr}}}}}

\newcommand\lse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
<\cr\simeq\cr}}}}}

\newcommand\gse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
>\cr\simeq\cr}}}}}

\newcommand\grole{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr
>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
>\cr\noalign{\vskip-1pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
>\cr\noalign{\vskip-0.5pt}<\cr}}}}}

\newcommand\leogr{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr
<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
<\cr\noalign{\vskip-1pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
<\cr\noalign{\vskip-0.5pt}>\cr}}}}}

\newcommand\loa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
<\cr\approx\cr}}}}}

\newcommand\goa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
>\cr\approx\cr}}}}}

\newcommand\sun{\hbox{$\odot$}}
\newcommand\earth{\hbox{$\oplus$}}
\newcommand\degr{\hbox{$^\circ$}}
\newcommand\diameter{{\ifmmode\mathchoice
{\ooalign{\hfil\hbox{$\reset@font\displaystyle/$}\hfil\crcr
{\hbox{$\reset@font\displaystyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\reset@font\textstyle/$}\hfil\crcr
{\hbox{$\reset@font\textstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\reset@font\scriptstyle/$}\hfil\crcr
{\hbox{$\reset@font\scriptstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\reset@font\scriptscriptstyle/$}\hfil\crcr
{\hbox{$\reset@font\scriptscriptstyle\mathchar"20D$}}}}
\else{\ooalign{\hfil/\hfil\crcr\mathhexbox20D}}%
\fi}}

\newcommand\sq{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}
\newcommand\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}

\newcommand{\romn}[1] {{\mathrm #1}}

%\newcommand\fd{\hbox{$.\!\!^{\reset@font\romn d}$}}
%\newcommand\fh{\hbox{$.\!\!^{\reset@font\romn h}$}}
%\newcommand\fm{\hbox{$.\!\!^{\reset@font\romn m}$}}
%\newcommand\fs{\hbox{$.\!\!^{\reset@font\romn s}$}}

\newcommand\fd{\hbox{$.\!\!^\mathrm{d}$}}
\newcommand\fh{\hbox{$.\!\!^\mathrm{h}$}}
\newcommand\fm{\hbox{$.\!\!^\mathrm{m}$}}
\newcommand\fs{\hbox{$.\!\!^\mathrm{s}$}}
\newcommand\fdg{\hbox{$.\!\!^\circ$}}
\newcommand\farcm{\hbox{$.\mkern-4mu^\prime$}}
\newcommand\farcs{\hbox{$.\!\!^{\prime\prime}$}}
\newcommand\fp{\hbox{$.\!\!^{\reset@font\reset@font\scriptscriptstyle\romn p}$}}
\newcommand\arcdeg{\hbox{$^\circ$}}
\newcommand\arcmin{\hbox{$^\prime\,$}}
\newcommand\arcsec{\hbox{$^{\prime\prime}$}}

\def\micron{\hbox{$\umu$m}}


% end of definitions


==> libbydefs.tex <==
% New Commands and Definitions

% Type styles

\newcommand{\sans}{\mdseries\sffamily\upshape}
\newcommand{\sansb}{\bfseries\sffamily\upshape}
\newcommand{\sansi}{\mdseries\sffamily\itshape}
\newcommand{\sansbi}{\bfseries\sffamily\itshape}
\newcommand{\sanssc}{\mdseries\sffamily\scshape}
\newcommand{\sansbsc}{\bfseries\sffamily\scshape}


% Units:

\newcommand{\cmpers}{\mbox{$\mathrm{cm\ s^{-1}}$}}
\newcommand{\cms}{\mbox{$\mathrm{cm^2}$}}
\newcommand{\cmspers}{\mbox{$\mathrm{cm^2\ s^{-1}}$}}
\newcommand{\ccpers}{\mbox{$\mathrm{cm^3\ s^{-1}}$}}
\newcommand{\percc}{\mbox{$\mathrm{cm^{-3}}$}}
\newcommand{\perccpers}{\mbox{$\mathrm{cm^{-3}\ s^{-1}}$}}
\newcommand{\kmpers}{\mbox{$\mathrm{km\ s^{-1}}$}}


% Various:

\newcommand{\zup}[1]{$^\mathrm{\,#1}$}
\newcommand{\x}{$\times$\ }
\newcommand{\etal}{\hbox{\it et al.\ }}
\newcommand{\ha}{H$\alpha$}
\newcommand{\ox}{[O{\sc iii}]}
\newcommand{\Av}{\mbox{$A_v$}}
\newcommand{\Ed}{\mbox{$E_\mathrm{D}$}}
\newcommand{\ISM}{\mbox{interstellar medium}}
\newcommand{\Vlsr}{\mbox{$V_\mathrm{LSR}$}}
\newcommand{\Lsol}{\hbox{L$_{\odot}$}}
\newcommand{\Msol}{\hbox{M$_{\odot}$}}
\newcommand{\Rsol}{\hbox{R$_{\odot}$}}


% Molecular Species:

\newcommand{\molh}{\mbox{$\mathrm{H_2}$}}
\newcommand{\Hp}{\mbox{$\mathrm{H^+}$}}
\newcommand{\Hep}{\mbox{$\mathrm{He^+}$}}
\newcommand{\HHHp}{\mbox{$\mathrm{H_3^+}$}}
\newcommand{\Cp}{\mbox{$\mathrm{C^+}$}}
\newcommand{\water}{\mbox{$\mathrm{H_2O}$}}
\newcommand{\CCH}{\mbox{$\mathrm{C_2H}$}}
\newcommand{\meth}{\mbox{$\mathrm{CH_3OH}$}}
\newcommand{\form}{\mbox{$\mathrm{H_2CO}$}}
\newcommand{\DDform}{\mbox{$\mathrm{D_2CO}$}}
\newcommand{\HCOp}{\mbox{$\mathrm{HCO^+}$}}
\newcommand{\ammo}{\mbox{$\mathrm{NH_3}$}}
\newcommand{\OO}{\mbox{$\mathrm{O_2}$}}
\newcommand{\HHD}{\mbox{$\mathrm{H_2D^+}$}}
\newcommand{\NNHp}{\mbox{$\mathrm{N_2H^+}$}}
\newcommand{\NND}{\hbox{N$_2$D$^+$}}


% Turbulence/Grains:

\newcommand{\Kz}{\mbox{$K=0$}}
\newcommand{\Ktwon}{\mbox{$K=10^{21}$}}
\newcommand{\Ktwtw}{\mbox{$K=10^{22}$}}
\newcommand{\Ktwth}{\mbox{$K=10^{23}$}}
\newcommand{\Tdis}{\mbox{$\tau_{dis}$}}
\newcommand{\Chieze}{Chi\`{e}ze}
\newcommand{\PdF}{Pineau des For\^{e}ts}
\newcommand{\vturb}{\mbox{$v_t$}}


% Objects:

%\newcommand{\IRAS}{\mbox{IRAS 16293-2422}}


% From Albert:

% \def\oversim#1#2{\lower0.5pt\vbox{\baselineskip0pt \lineskip-0.5pt 
%                  \ialign{$\mathsurround0pt #1\hfil##\hfil$\crcr#2\crcr\sim\crcr}}}
% \def\gsim{\mathrel{\mathpalette\oversim>}}    % > over \sim
% \def\lsim{\mathrel{\mathpalette\oversim<}}    % < over \sim

% \newcommand{\note}[1]{{\bf [#1]}}

% note at end 
\def\thisrep{\vspace{0.5cm}\normalsize\noindent 
	     This report has been typeset from a \TeX\ / \LaTeX\ file prepared by the author.}
\def\thisshow{\vspace{0.5cm}\normalsize\noindent 
	     This slide show has been typeset from a \TeX\ / \LaTeX\ file prepared by the author.}

% end of file


